Localized Manifold Harmonics for Spectral Shape Analysis

The use of Laplacian eigenfunctions is ubiquitous in a wide range of computer graphics and geometry processing applications. In particular, Laplacian eigenbases allow generalizing the classical Fourier analysis to manifolds. A key drawback of such bases is their inherently global nature, as the Laplacian eigenfunctions carry geometric and topological structure of the entire manifold. In this paper, we introduce a new framework for local spectral shape analysis. We show how to efficiently construct localized orthogonal bases by solving an optimization problem that in turn can be posed as the eigendecomposition of a new operator obtained by a modification of the standard Laplacian. We study the theoretical and computational aspects of the proposed framework and showcase our new construction on the classical problems of shape approximation and correspondence. We obtain significant improvement compared to classical Laplacian eigenbases as well as other alternatives for constructing localized bases.

==> supmat <==
\newpage
\section{Supplementary Material}
These pages contain proofs for Theorems 1 and 2 appearing in the main paper \cite{lmh}.

\paragraph*{Proof of Theorem 1. }
%
Let $ \mathbf{W} $,  $ \mu_{\bot}\mathbf{A}\mathbf{P}_{k'} $ and $ \mu_{R}\mathbf{A}\mathrm{diag}(\mathbf{v}) $ be real symmetric positive semidefinite matrices of dimension $ n \times n$, and define $\Q_{v,k'} = \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}+ \mu_{R}\mathbf{A}\mathrm{diag}(\mathbf{v}) $.
Let $ 0 = \lambda_{1}(\mathbf{W}) \leq \ldots \leq \lambda _{n} (\mathbf{W})$ be the eigenvalues for the generalized eigenvalue problem of $\mathbf{W}$ and $ \lambda_{1}( \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) \leq \ldots \leq \lambda _{n}( \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})$ and $ \lambda_{1}(\Q_{v,k'}) \leq \ldots \leq \lambda _{n}(\Q_{v,k'})$ be the generalized eigenvalues of $  \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'} $ and $\Q_{v,k'}$ respectively.
We aim to prove that 
%
\begin{equation}
\lambda _{k'}(\mathbf{W}) \le \lambda _1(\Q_{v,k'}) \,,
\end{equation}
%
for some $\mu_{\bot} , \mu_{R} \in \mathbb{R}$ and for every $k' \in \left\lbrace 0, \ldots , n-1 \right\rbrace$.

We start by observing that
\begin{equation}\label{r1}
\lambda _{k'}(\mathbf{W}) \leq \lambda _{k'+1}(\mathbf{W}) = \lambda _{1}( \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\,,
\end{equation}
%
where the first inequality is given by the non-decreasing ordering of the eigenvalues, and the equality on the right follows from the fact that for some choice of $\mu_{\bot}> \lambda _{k'+1}(\mathbf{W})$, $\bm{\phi}_{k'+1}$ is the minimizer of $\mathbf{x}^{\top}( \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x}$ under the orthogonality conditions $\left\langle \mathbf{x}, \mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1$ and $\left\langle \bm{\phi} _{l}, \mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 0$, $\forall l \in \left\lbrace 1, \ldots , k' \right\rbrace $, i.e., $( \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} = \mathbf{0}$.
%
%Indeed, from the definition of eigenfunction $\bm{\phi}_{k'+1}$ is the vector with norm equal to $1$ and orthogonal to $\bm{\phi}_{l} \ \forall l \in \left\lbrace 1, \ldots , k' \right\rbrace $ which minimize $\mathbf{x}^{\top}(\mathbf{W})\mathbf{x}$.

Invoking a special case of Corollary 4.3.4b in \cite{horn2012matrix} and using the fact that $\mu_{R}\mathbf{A}\mathrm{diag}(\mathbf{v})$ only has non-negative eigenvalues (being a diagonal matrix with non-negative entries), we obtain the following inequality:
%
\begin{equation}\label{r2}
\lambda _{1}( \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) \leq \lambda _{1}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) + \mu_{R}\mathbf{A}\mathrm{diag}(\mathbf{v})) = \lambda _{1}(\Q_{v,k'}) \,.
\end{equation}
%
Furthermore, this inequality is an equality if and only if $\exists \mathbf{x} \in \mathbb{R}^{n}$ s.t. $\mathbf{x} \neq 0$ and the following three conditions are satisfied:
\begin{enumerate}
\item $( \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} = \lambda _{1}( \mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} $;
\item $(\Q_{v,k'})\mathbf{x} = \lambda _{1}(\Q_{v,k'})\mathbf{x} $;
\item $(\mu_{R}\mathbf{A}\mathrm{diag}(\mathbf{v}))\mathbf{x} = 0 $.
\end{enumerate}
%The last condition means that the integral of the eigenfunction $x$ restricted to the part of the surface $\mathcal{X}$ complementary to $u$ is equal to $0$.
%
Putting together \eqref{r1} and \eqref{r2} we can conclude that:
%
\begin{equation}
\lambda _{k'}(\mathbf{W}) \le \lambda _{k'+1}(\mathbf{W}) \le \lambda _1(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) \le \lambda _1(\Q _{v,k'})\,.
\end{equation}
%
Note that the existence of a gap is given either by the violation of any of the three conditions above, or in the presence of simple spectra, i.e., whenever $\lambda _{k'}(\mathbf{W}) \neq \lambda _{k'+1}(\mathbf{W})$.
%

\paragraph*{Choice of $\mu_{\bot}$.}
%
%$ \mathbf{W} $ and $ \mu_{\bot}\mathbf{P}_{k'} $ are real symmetric positive semidefinite matrices of dimension $ n \times n$. Let $ 0 = \lambda_{1}(\mathbf{W}) \leq \ldots \leq \lambda _{n} (\mathbf{W})$ the eigenvalues of the generalized eigenvalue problem of $\mathbf{W}$ and $ \lambda_{1}( \mathbf{W} + \mu_{\bot}\mathbf{P}_{k'}) \leq \ldots \leq \lambda _{n}( \mathbf{W} + \mu_{\bot}\mathbf{P}_{k'})$ the generalized eigenvalues of $  \mathbf{W} + \mu_{\bot}\mathbf{P}_{k'} $.
We aim to prove that for every $\mu_{\bot} > \gamma$ for some $\gamma \in \mathbb{R}^{+}$ we have:
%
\begin{equation}
\lambda_{1}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) \geq \lambda_{k'+1}(\mathbf{W} ) \,.
\end{equation}
%
We can rewrite the two terms of this inequality as:
%
\begin{align}
\lambda_{1}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) &= \underset{\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1}{\min} \mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} \label{t1}\\
\lambda_{k'+1}(\mathbf{W} ) &= \underset{\underset{\left\langle \bm{\phi} _{i}, \mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 0, \ \forall i = 1, \ldots, k' }{\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1}}{\min} \mathbf{x}^{\top}\mathbf{W}\mathbf{x} \,.
\end{align}
%
The objective in \eqref{t1} can be rewritten as:
%
\begin{equation}\label{sums}
\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} =  \mathbf{x}^{\top}\mathbf{W}\mathbf{x} + \mathbf{x}^{\top}(\mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} \,.
\end{equation}
%
We now express our vectors as the Fourier series $\mathbf{x} = \sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i}$, where $\alpha _{i} = \left\langle \bm{\phi}_i,\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})}$. Noting that $\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1 $ implies $\sum_{i=1}^{n}\alpha_{i}^2 = 1$, we can write:
%
\begin{equation}\label{rr1}
\mathbf{x}^{\top}\mathbf{W}\mathbf{x} = (\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i})^{\top}\mathbf{W}(\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i}) = (\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i})^{\top}(\sum_{i=1}^{n}\lambda_{i}(\mathbf{W})\alpha _{i} \mathbf{A}\bm{\phi}_{i}) = \sum_{i=1}^{n}\lambda_{i}(\mathbf{W})\alpha _{i}^2 \,.
\end{equation}
%
Similarly, we can rewrite the second summand in \eqref{sums} as:
%
\begin{align}
\mathbf{x}^{\top}(\mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} &= (\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i})^{\top}(\mu_{\bot}\mathbf{A}\mathbf{P}_{k'})(\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i})\\
& = \mu_{\bot}(\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i})^{\top}(\mathbf{A}\bm{\Phi}\bm{\Phi}^{\top}\mathbf{A})(\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i}) \\
&= \mu_{\bot}\Big((\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i})^{\top}\mathbf{A}\bm{\Phi}\Big) \Big(\bm{\Phi}^{\top}\mathbf{A}(\sum_{i=1}^{n}\alpha _{i} \bm{\phi}_{i})\Big)\\
& = \mu_{\bot}\left[ \alpha_{1} , \ldots , \alpha_{k'} \right] \left[\alpha_{1} , \ldots , \alpha_{k'} \right] ^{\top}\\
& = \mu_{\bot}\sum_{i=1}^{k'}\alpha _{i}^2 \label{rr2}\,.
\end{align}
%
From \eqref{rr1} and \eqref{rr2} we can conclude:
%
\begin{equation}
\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} = \mathbf{x}^{\top}\mathbf{W}\mathbf{x} + \mathbf{x}^{\top}(\mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} = \sum_{i=1}^{n}\lambda_{i}(\mathbf{W})\alpha _{i}^2 + \mu_{\bot}\sum_{i=1}^{k'}\alpha _{i}^2 \,.
\end{equation}
%
At this point we split the proof in three different cases:
%
\begin{enumerate}
\item $\left\langle \bm{\phi} _{i}, \mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 0, \ \forall i = 1, \ldots, k' $, that is equivalent to ask that $\mathbf{P}_{k'}\mathbf{x} = \mathbf{0}$. In this case we have:
%
\begin{align}
\lambda_{1}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) &= \underset{\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1}{\min} \mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} \\
&=\underset{\underset{\left\langle \bm{\phi} _{i}, \mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 0, \ \forall i = 1, \ldots, k' }{\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1}}{\min} (\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x}) \\
&=
\underset{\underset{\left\langle \bm{\phi} _{i}, \mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 0, \ \forall i = 1, \ldots, k' }{\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1}}{\min} \mathbf{x}^{\top}\mathbf{W}\mathbf{x} = \lambda_{k'+1}(\mathbf{W} )\,.
\end{align}
%
\item $\mathbf{x} \in span(\bm{\phi}_{1}, \ldots , \bm{\phi}_{k'})$, implying that $\alpha_{i} = 0 \ \forall i > k'$ and hence $\mathbf{x} = \sum_{i=1}^{k'}\alpha _{i} \bm{\phi}_{i}$. We get:
%
\begin{equation}
\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} = \sum_{i=1}^{k'}\lambda_{i}(\mathbf{W})\alpha _{i}^2 + \mu_{\bot}\sum_{i=1}^{k'}\alpha _{i}^2 \,.
\end{equation}
%
Since we take the minimum over the $\mathbf{x}$ s.t. $\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1$ we have $\sum_{i=1}^{k'}\alpha _{i}^2 = 1 $ and:
%
\begin{equation}
\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} = \sum_{i=1}^{k'}\lambda_{i}(\mathbf{W})\alpha _{i}^2 + \mu_{\bot} \geq \mu_{\bot}  \,,
\end{equation}
%
where the equality is realized for $\mathbf{x} = \bm{\phi}_{1}$ since $\lambda_{1}(\mathbf{W}) = 0$, and all other cases yield $\mu_{\bot}$ plus some non-negative quantity. We get to:
%
\begin{equation}
\lambda_{1}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) = \underset{\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1}{\min} \mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} = \mu_{\bot} \,.
\end{equation}
%
\item For the last case we have $\left\langle \bm{\phi} _{i}, \mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} \neq 0 $ for at least one $i = 1, \ldots , k'$   and for at least one $i > k'$ at the same time. 
%
\begin{align}
\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} &= \sum_{i=1}^{n}\lambda_{i}(\mathbf{W})\alpha _{i}^2 + \mu_{\bot}\sum_{i=1}^{k'}\alpha _{i}^2 \\
&= \sum_{i=1}^{k'}\lambda_{i}(\mathbf{W})\alpha _{i}^2 + \sum_{i=k'+1}^{n}\lambda_{i}(\mathbf{W})\alpha _{i}^2 + \mu_{\bot}\sum_{i=1}^{k'}\alpha _{i}^2 \\&= \sum_{i=1}^{k'}(\lambda_{i}(\mathbf{W}) + \mu_{\bot})\alpha _{i}^2 + \sum_{i=k'+1}^{n}\lambda_{i}(\mathbf{W})\alpha _{i}^2 \,.
\end{align}
%
Since $\lambda_{i}(\mathbf{W}) \geq \lambda_{k'+1}(\mathbf{W})$, $\forall i \geq k'+1$ we can write:
%
\begin{align}
\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} &= \sum_{i=1}^{k'}(\lambda_{i}(\mathbf{W}) + \mu_{\bot})\alpha _{i}^2 + \sum_{i=k'+1}^{n}\lambda_{i}(\mathbf{W})\alpha _{i}^2 \\
&\geq
 \sum_{i=1}^{k'}(\lambda_{i}(\mathbf{W}) + \mu_{\bot})\alpha _{i}^2 + \lambda_{k'+1}(\mathbf{W})\sum_{i=k'+1}^{n}\alpha _{i}^2\\&\geq
\sum_{i=1}^{k'}\mu_{\bot}\alpha _{i}^2 + \lambda_{k'+1}(\mathbf{W})\sum_{i=k'+1}^{n}\alpha _{i}^2
\,.
\end{align}
%
If we take $\mu_{\bot} > \lambda_{k'+1}(\mathbf{W}) $ in order to satisfy the condition imposed by case 2, we get:
%
\begin{align}
\mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} &\geq
\sum_{i=1}^{k'}\mu_{\bot}\alpha _{i}^2 + \lambda_{k'+1}(\mathbf{W})\sum_{i=k'+1}^{n}\alpha _{i}^2 \\
&> \lambda_{k'+1}(\mathbf{W})\sum_{i=1}^{k'}\alpha _{i}^2 + \lambda_{k'+1}(\mathbf{W})\sum_{i=k'+1}^{n}\alpha _{i}^2 \\&= \lambda_{k'+1}(\mathbf{W})\sum_{i=1}^{n}\alpha _{i}^2\\& = \lambda_{k'+1}(\mathbf{W})
\,.
\end{align}
%
We can therefore conclude that
%
\begin{equation}
\lambda_{1}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) = \underset{\left\langle \mathbf{x},\mathbf{x} \right\rangle _{L^{2}(\mathcal{X})} = 1}{\min} \mathbf{x}^{\top}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})\mathbf{x} > \lambda_{k'+1}(\mathbf{W}) \ \mathit{if} \ \mu_{\bot} > \lambda_{k'+1}(\mathbf{W})\,.
\end{equation}
%
\end{enumerate}
%
In Figure \ref{fig:etas} we show an empirical evaluation across several choices of $\mu _{\bot}$.
\begin{figure}[bt]
  \centering
  \input{etas.tikz}
  \caption{\label{fig:etas}Plot of $\lambda_{1}(\mathbf{W} + \mu_{\bot}\mathbf{A}\mathbf{P}_{k'})$ at increasing $\mu_{\bot}$. Note how for every $\mu_{\bot} \leq \lambda_{k'+1}(\mathbf{W})$ the frequency ($y$-axis) increases, converging at $\mu_{\bot} >\lambda_{k'+1}(\mathbf{W})$. At convergence, the orthogonality constraint (encoded in the penalty term $\mathcal{E}_\bot(\psi)$ in the LMH formulation) is satisfied.}
\end{figure}
%
%\paragraph*{B - Proof of Theorem 2. }
%We give only an idea of how this Theorem can be proved. 
%First of all we remark that the behaviour suggested in the Theorem 2 is widely observed empirically (please refer to Figure 2 and Figure 3 in the main document).
%Now if we select $\mu_{\bot} = 0 $ and $ \mu_{R} \gg 0$, as observed in Section 5, we obtain exactly the harmonics computed on the partial surface extracted from the region $R \subseteq \mathcal{X}$.
%In this case we clearly gain the Weyl's asymptotic law for the eigenvalues of $\Q _{v,k'}$.
%Now if $\mu_{R}$ is sufficiently large to ensure the localization of the Local Manifold Harmonics in the region $R$, the behaviour of the eigenvalues is the one suggested.
%The limited variations could be due to the orthogonality constraint imposed.
%We observed that this constraint moves slightly the eigenvalues in order to ensure the required condition, and does not damage the expected growth.
%
\paragraph*{Proof of Theorem 2. }
We want to show that $\forall k \in \left\lbrace 1, 2, \ldots ,n \right\rbrace $ we have the following upper bound:
$$ \lambda _{i}(\Q _{v,k'}) \leq \lambda_{i+k'}(\mathbf{W}^{R}) \ .$$
Similarly to Theorem 1, the proof follows directly from Corollary 4.3.4b in \cite{horn2012matrix}, which specialized to our case reads:
%
\begin{equation} 
\lambda _{i}(\mathbf{W}^{R}+\mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) \leq \lambda_{i+\pi}(\mathbf{W}^{R})\,,
\end{equation}
where $\pi$ is the number of positive eigenvalues of $\mu_{\bot}\mathbf{A}\mathbf{P}_{k'}$. Since $\Q _{v,k'} = \mathbf{W}^{R}+\mu_{\bot}\mathbf{A}\mathbf{P}_{k'}$ and using the fact that $\mu_{\bot}\mathbf{A}\mathbf{P}_{k'}$ is a positive semidefinite matrix with rank $k'$, we have $\pi=k'$, leading to:
\begin{equation}
\lambda _{i}(\Q _{v,k'}) = \lambda _{i}(\mathbf{W}^{R}+\mu_{\bot}\mathbf{A}\mathbf{P}_{k'}) \leq \lambda_{i+\pi}(\mathbf{W}^{R}) = \lambda_{i+k'}(\mathbf{W}^{R})\,.
\end{equation}


%
%\bibliographystyle{eg-alpha-doi}
% \bibliographystyle{plain}
% \bibliography{egbib}
%
